SplatMesh: Interactive 3D Segmentation and Editing Using Mesh-Based Gaussian Splatting

A key challenge in fine-grained 3D-based interactive editing is the absence of an efficient representation that balances diverse modifications with high-quality view synthesis under a given memory constraint. While 3D meshes provide robustness for various modifications, they often yield lower-quality view synthesis compared to 3D Gaussian Splatting, which, in turn, suffers from instability during extensive editing. A straightforward combination of these two representations results in suboptimal performance and fails to meet memory constraints. In this paper, we introduce SplatMesh, a novel fine-grained interactive 3D segmentation and editing algorithm that integrates 3D Gaussian Splat with a precomputed mesh and could adjust the memory request based on the requirement. Specifically, given a mesh, \method simplifies it while considering both color and shape, ensuring it meets memory constraints. Then, SplatMesh aligns Gaussian splats with the simplified mesh by treating each triangle as a new reference point. By segmenting and editing the simplified mesh, we can effectively edit the Gaussian splats as well, which will lead to extensive experiments on real and synthetic datasets, coupled with illustrative visual examples, highlighting the superiority of our approach in terms of representation quality and editing performance. Code of our paper can be found here: https://github.com/kaichen-z/SplatMesh.

==> sec/5_sup.tex <==

\begin{figure*}[tbhp]
    \centering
    \includegraphics[width=0.8\linewidth, clip]{figures/dtu_res.pdf}
    \caption{\textbf{Qualitative Comparison of View Synthesis on DTU Dataset.}
    Note SuGaR uses a different mesh extraction strategy from ours, so it includes some background.
    }
    \vspace{-0.3cm}
    \label{fig:dtu_results}
\end{figure*}


\input{tables/tab_dtu}










==> tables/tab_abl.tex <==
\begin{table}[tb]

  \vspace{-4pt}
  \label{tab:nvos}
  \centering
  \begin{tabular}{lccc}
    \toprule
    Method     & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
    \midrule
    \method (K=4) & 30.487 & 0.944 & 0.060 \\
    \method (w/o $n_s$) &31.150 & 0.951 & 0.043\\
    \method (w/o $n_r$) & 31.413 & 0.952 & 0.041\\
    \method (K=8) & \textbf{31.701} & \textbf{0.954} & \textbf{0.037} \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Quantitative Results of Ablation Studies for \method on NeRF Synthetic.}}
  \label{table.segment}
\end{table}

==> tables/tab_mesh.tex <==
\begin{table*}[tb]
\centering
\resizebox{1.0\linewidth}{!}{
\tabcolsep 3pt
\begin{tabular}{lcccccccccccccccc}
\toprule
 & \multicolumn{16}{c}{DTU Scan ID} \\ \midrule
Method & \multicolumn{1}{r}{24} & \multicolumn{1}{r}{37} & \multicolumn{1}{r}{40} & \multicolumn{1}{r}{55} & \multicolumn{1}{r}{63} & \multicolumn{1}{r}{65} & \multicolumn{1}{r}{69} & \multicolumn{1}{r}{83} & \multicolumn{1}{r}{97} & \multicolumn{1}{r}{105} & \multicolumn{1}{r}{106} & \multicolumn{1}{r}{110} & \multicolumn{1}{r}{114} & \multicolumn{1}{r}{118} & \multicolumn{1}{r}{122} & \multicolumn{1}{r}{Avg.} \\ \midrule
NeuTex~\cite{xiang2021neutex} & 2.078 & 5.038 & 3.477 & 1.039 & 3.744 & 2.078 & 3.201 & 2.163 & 5.104 & 1.828 & 1.951 & 4.319 & 1.177 & 3.100 & 1.921 & 2.815  \\
NeuS~\cite{wang2021neus} & 1.544 & 1.224 & 1.065 & 0.665 & 1.286 & 0.825 & 0.904 & 1.350 & 1.320 & 0.855 & 0.987 & 1.328 & 0.487 & 0.636 & 0.678 & 1.010 \\
NeuMesh~\cite{neumesh} & 1.112 & 1.262 & 0.988 & 0.674 & 1.224 & 0.835 & \textbf{0.878} & 1.232 & 1.304 & 0.741 & 0.963 & 1.239 & 0.558 & 0.645 & 0.739 & 0.960  \\
Ours & \textbf{1.038} & \textbf{1.213} & \textbf{0.979} & \textbf{0.656} & \textbf{1.222} & \textbf{0.817} & 0.898 & \textbf{1.150} & \textbf{1.296} & \textbf{0.732} & \textbf{0.946} & \textbf{1.190} & \textbf{0.468} & \textbf{0.625} & \textbf{0.651} & \textbf{0.942}
 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitative Results for Mesh Reconstruction on DTU.}
We compare mesh quality using Chamfer distance on the DTU dataset.
We use training split of images instead of full images, so the result of NeuS~\cite{wang2021neus} is different from the original paper.
}
\vspace{-0.5cm}
\label{tab:mesh}
\end{table*}



==> tables/tab_render.tex <==
\begin{table*}[tb]
\centering
\resizebox{0.85\linewidth}{!}{
\tabcolsep 13pt
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{DTU} & \multicolumn{3}{c}{NeRF 360$^{\circ}$ Synthetic} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}  
\multicolumn{1}{c}{} & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} & \multicolumn{1}{l}{PSNR $\uparrow$} & \multicolumn{1}{l}{SSIM $\uparrow$} & \multicolumn{1}{l}{LPIPS $\downarrow$} \\ 
\hline
NeuTex~\cite{xiang2021neutex} & 26.080 & 0.893 & 0.196 & 25.718 & 0.914 & 0.109 \\
NeuS~\cite{wang2021neus} & 26.352 & 0.909 & 0.176 & 30.588 & \textbf{0.960} & 0.058 \\
NeuMesh~\cite{neumesh} & 28.289 & 0.921 & \textbf{0.117} & 30.945 & 0.951 & 0.043 \\
Ours & \textbf{29.113} & \textbf{0.924} & 0.121 & \textbf{31.701} & 0.954 & \textbf{0.037} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitative Results for View Synthesis on DTU and NeRF Synthetic.} Our method achieves the best performance while enabling interactive segmentation and editing on both two datasets.}
\label{tab:View Synthesis}
\vspace{-0.5cm}
\end{table*}

==> tables/tab_seg.tex <==
\begin{table}[tb]
  \vspace{-4pt}
  \label{tab:nvos}
  \centering
  \begin{tabular}{lccc}
    \toprule
    Method     & mIoU (\%)& Acc (\%) & Tuning \\
    \midrule
    NVOS~\cite{nvos} & 70.1  & 92.0 & $\checkmark$ \\
    SA3D~\cite{cen2023segment} & \textbf{90.3} & \textbf{98.2} & $\checkmark$ \\
    % \hline
    Graph-Cut (3D)~\cite{GrabCut} & 39.4 & 73.6 &  \\
    ISRF~\cite{isrf} & 83.8 & 96.4 &  \\
    % \hline
    Ours & \textbf{90.3} & 97.6 & \\
    \bottomrule
  \end{tabular}
  \vspace{-7pt}
    \caption{\textbf{Quantitative Results for 3D Segmentation on NVOS in terms of mIoU (Intersection-Over-Union) and Accuracy.} 
  % We compare the mIoU and accuracy with Graph-Cut (3D)~\cite{GrabCut}, NVOS~\cite{nvos}, ISRF~\cite{isrf} and SA3D~\cite{cen2023segment}. 
  Tuning refers to whether fine-tuning is necessary for the model when presented with new prompts.
  }
  \vspace{-9pt}
  \label{table.segment}
\end{table}
